3D-0D closed-loop model for the simulation of cardiac biventricular electromechanics

Two crucial factors for accurate numerical simulations of cardiac electromechanics, which are also essential to reproduce the synchronous activity of the heart, are: i) accounting for the interaction between the heart and the circulatory system that determines pressures and volumes loads in the heart chambers; ii) reconstructing the muscular fiber architecture that drives the electrophysiology signal and the myocardium contraction. In this work, we present a 3D biventricular electromechanical model coupled with a 0D closed-loop model of the whole cardiovascular system that addresses the two former crucial factors. With this aim, we introduce a boundary condition for the mechanical problem that accounts for the neglected part of the domain located on top of the biventricular basal plane and that is consistent with the principles of momentum and energy conservation. We also discuss in detail the coupling conditions that stand behind the 3D and the 0D models. We perform electromechanical simulations in physiological conditions using the 3D-0D model and we show that our results match the experimental data of relevant mechanical biomarkers available in literature. Furthermore, we investigate different arrangements in cross-fibers active contraction. We prove that an active tension along the sheet direction counteracts the myofiber contraction, while the one along the sheet-normal direction enhances the cardiac work. Finally, several myofiber architectures are analysed. We show that a different fiber field in the septal area and in the transmural wall effect the pumping functionality of the left ventricle.

==> EMmodel_biv_CMAME.tex <==
% This block of code is essential to use the [resume] flag for subequations
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\makeatletter
\def\user@resume{resume}
\def\user@intermezzo{intermezzo}
%
\newcounter{previousequation}
\newcounter{lastsubequation}
\newcounter{savedparentequation}
\setcounter{savedparentequation}{1}
%
\renewenvironment{subequations}[1][]{%
	\def\user@decides{#1}%
	\setcounter{previousequation}{\value{equation}}%
	\ifx\user@decides\user@resume
	\setcounter{equation}{\value{savedparentequation}}%
	\else
	\ifx\user@decides\user@intermezzo
	\refstepcounter{equation}%
	\else
	\setcounter{lastsubequation}{0}%
	\refstepcounter{equation}%
	\fi\fi
	\protected@edef\theHparentequation{%
		\@ifundefined {theHequation}\theequation \theHequation}%
	\protected@edef\theparentequation{\theequation}%
	\setcounter{parentequation}{\value{equation}}%
	\ifx\user@decides\user@resume
	\setcounter{equation}{\value{lastsubequation}}%
	\else
	\setcounter{equation}{0}%
	\fi
	\def\theequation  {\theparentequation  \alph{equation}}%
	\def\theHequation {\theHparentequation \alph{equation}}%
	\ignorespaces
}{%
	%  \arabic{equation};\arabic{savedparentequation};\arabic{lastsubequation}
	\ifx\user@decides\user@resume
	\setcounter{lastsubequation}{\value{equation}}%
	\setcounter{equation}{\value{previousequation}}%
	\else
	\ifx\user@decides\user@intermezzo
	\setcounter{equation}{\value{parentequation}}%
	\else
	\setcounter{lastsubequation}{\value{equation}}%
	\setcounter{savedparentequation}{\value{parentequation}}%
	\setcounter{equation}{\value{parentequation}}%
	\fi\fi
	%  \arabic{equation};\arabic{savedparentequation};\arabic{lastsubequation}
	\ignorespacesafterend
}
\makeatother
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\newlength{\temp}
\newcommand{\EPfirstline}{
	J \EPchim \left[ \EPCm \dfrac{\partial u}{\partial t} + \EPIion(u, \boldsymbol{w}) \right] - \nabla \cdot ( J \mecF^{-1} \EPdiffTens \, \mecF^{-T} \nabla u) = J \EPchim \EPIapp(t)
}
\settowidth{\temp}{$\EPfirstline$}
\newcommand{\widthbox}[1]{\makebox[\temp][l]{$#1$}}

\begin{subequations}\label{eqn: EM}
	\renewcommand{\theequation}{\theparentequation.\arabic{equation}}
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	%(EP)
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	\begin{empheq}[left={(\PhyEP)\empheqlbrace\,}]{align}
		& \EPfirstline & \text{in } \Omega_0 \times (0,T], \label{eqn: EP1}\\
		& \widthbox{\dfrac{\partial \boldsymbol{w}}{\partial t} - \EPrhsGating(u, \boldsymbol{w}) = \boldsymbol{0}} & \text{in } \Omega_0 \times (0,T], \label{eqn: EP2}\\
		& \left( J \mecF^{-1} \EPdiffTens \, \mecF^{-T} \nabla u \right) \cdot \mecNref = 0  & \text{on } \partial \Omega_0 \times (0, T] \label{eqn: EP3},
	\end{empheq}
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	%(A)
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	\begin{empheq}[left={(\PhyAct)\empheqlbrace\,}]{align}
		\quad \widthbox{ \frac{\partial \ActStateHF}{\partial t} = \ActRhs(\ActStateHF,\Cai,\SL) } & \text{in } \Omega_0 \times (0,T] \label{eqn: Act},
	\end{empheq}
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	% (M)
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	\begin{empheq}[left={(\PhyMec)\empheqlbrace\,}]{align}
		& \widthbox{\rho_{\text{s}} \dfrac{\partial^2 \displ}{\partial t^2} - \nabla \cdot \tenspiola(\displ, \Tens(\ActStateHF)) = \boldsymbol{0} }
		%\qquad
		&\text{in } \Omega_0 \times (0,T], \label{eqn: Mec1}\\
		& \tenspiola(\displ, \Tens(\ActStateHF)) \mecNref = \BCmecKepiTens \displ +
		\BCmecCepiTens \dfrac{\partial \displ}{\partial t}
		%\qquad \qquad \qquad \qquad \qquad \qquad \qquad \, \,
		&\text{on } \GammaEpi \times (0, T], \label{eqn: Mec2}\\
		&\tenspiola(\displ, \Tens(\ActStateHF)) \mecNref = -\PLV(t) \, J \mecF^{-T} \mecNref 	
		%\qquad \qquad \qquad \qquad \qquad \qquad \, \, \,
		&\text{on }\GammaEndoLV \times (0, T], \label{eqn: Mec3}\\
		& \tenspiola(\displ, \Tens(\ActStateHF)) \mecNref = -\PRV(t) \, J \mecF^{-T} \mecNref
		%\qquad \qquad \qquad \qquad \qquad \qquad \, \,
		&\text{on } \GammaEndoRV \times (0, T], \label{eqn: Mec4}\\
		& \tenspiola(\displ, \Tens(\ActStateHF)) \mecNref = \displaystyle | J \mecF^{-T} \mecNref | \left[ \PLV(t)\BCmecVbaseLV(t,\XiHat) + \PRV(t)\BCmecVbaseRV(t,\XiHat) \right] 
		%\: \, \,
		&\text{on } \GammaBase \times (0, T] \label{eqn: Mec5},
		%in $\Omega_0 \times (0, T)$, with $\displ = \displ_0$ and $\dfrac{\partial \displ}{\partial t} = \Dot{\displ}_0$ in $\Omega_0$ at time $t=0$.
	\end{empheq}
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	% (C)
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	\begin{empheq}[left={(\PhyCirc)\empheqlbrace\,}]{align} \label{eqn: Circ}
		\widthbox{\dfrac{d \Circ(t)}{d t} = \CircRhs(t, \Circ(t), \PLV(t), \PRV(t)) } & \text{for } t \in (0,T],
	\end{empheq}
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	% (V)
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	\begin{empheq}[left={(\PhyCoupl)\empheqlbrace\,}]{align}
		\widthbox{\VLV(\Circ(t)) = \VLVthreedim(\displ(t)) } & \text{for } t \in (0,T], \label{eqn: Coupl1}\\
		\widthbox{\VRV(\Circ(t)) = \VRVthreedim(\displ(t)) } & \text{for } t \in (0,T]. \label{eqn: Coupl2}
	\end{empheq}
\end{subequations}

==> pictures/header_slides.tex <==
\RequirePackage[T1]{fontenc}
\PassOptionsToPackage{sfdefault, lining}{FiraSans}
\RequirePackage{FiraSans}

\usepackage{sfmath} % to force sans serif in math mode
\renewcommand{\familydefault}{\sfdefault} % per usare il sans serif nel testo

\usepackage{amssymb}
\usepackage{bbm} %per la funzione indicatrice
\usepackage{mathrsfs} %per mathscr

\usepackage{xcolor}
%\usepackage{siunitx} 
%\usepackage{tabularx}

\input{../macros.tex}
